Rotationally Driven Ultraviolet Emission of Red Giant Stars

Main sequence stars exhibit a clear rotation-activity relationship, in which rapidly rotating stars drive strong chromospheric/coronal ultraviolet and X-ray emission. While the vast majority of red giant stars are inactive, a few percent exhibit strong ultraviolet emission. Here we use a sample of 133 red giant stars observed by SDSS APOGEE and GALEX to demonstrate an empirical relationship between NUV excess and rotational velocity (vsini). Beyond this simple relationship, we find that NUV excess also correlates with rotation period and with Rossby number in a manner that shares broadly similar trends to those found in M dwarfs, including activity saturation among rapid rotators. Our data also suggest that the most extremely rapidly rotating giants may exhibit so-called "super-saturation", which could be caused by centrifugal stripping of these stars rotating at a high fraction of breakup speed. As an example application of our empirical rotation-activity relation, we demonstrate that the NUV emission observed from a recently reported system comprising a red giant with a black hole companion is fully consistent with arising from the rapidly rotating red giant in that system. Most fundamentally, our findings suggest a common origin of chromospheric activity in rotation and convection for cool stars from main sequence to red giant stages of evolution.

==> All_Giants_Corr.tex <==
\begin{table*}
    \centering
        \begin{tabular}{lrrrrrrr}
        \toprule
        {} &  NUV\_exess &     vsini &     psini &      mass &    radius &       M\_H &       C\_N \\
        \midrule
        NUV\_exess &   1.000000 & -0.332996 &  0.384667 & -0.044692 &  0.177530 &  0.290217 & -0.071597 \\
        vsini     &  -0.332996 &  1.000000 & -0.781493 &  0.099516 & -0.081504 & -0.140155 &  0.137003 \\
        psini     &   0.384667 & -0.781493 &  1.000000 & -0.015873 &  0.300011 &  0.195655 & -0.109648 \\
        mass      &  -0.044692 &  0.099516 & -0.015873 &  1.000000 &  0.428797 &  0.193628 & -0.216819 \\
        radius    &   0.177530 & -0.081504 &  0.300011 &  0.428797 &  1.000000 &  0.210289 & -0.029044 \\
        M\_H       &   0.290217 & -0.140155 &  0.195655 &  0.193628 &  0.210289 &  1.000000 & -0.232016 \\
        C\_N       &  -0.071597 &  0.137003 & -0.109648 & -0.216819 & -0.029044 & -0.232016 &  1.000000 \\
        \bottomrule
        \end{tabular}
   \caption{Kendall correlation matrix of parameters checked for interdependence. *Note matrix is formed from giants with derived p/sini values only}
\end{table*}


==> Full_Giants_Corr.tex <==
\begin{table*}
    \centering
        \begin{tabular}{lrrrrrrrrr}
        \toprule
        {} &  NUV\_exess &     vsini &     psini &         T &      logg &      mass &    radius &       M\_H &       C\_N \\
        \midrule
        NUV\_exess &   1.000000 & -0.435463 &  0.396239 &  0.201553 & -0.323136 & -0.051003 &  0.170720 &  0.237106 & -0.074333 \\
        vsini     &  -0.435463 &  1.000000 & -0.779886 & -0.306335 &  0.290338 &  0.093094 & -0.092749 & -0.099701 &  0.153920 \\
        psini     &   0.396239 & -0.779886 &  1.000000 & -0.044333 & -0.436030 & -0.008223 &  0.312863 &  0.196941 & -0.105284 \\
        T         &   0.201553 & -0.306335 & -0.044333 &  1.000000 &  0.048937 &  0.102524 & -0.133690 & -0.099383 & -0.184950 \\
        logg      &  -0.323136 &  0.290338 & -0.436030 &  0.048937 &  1.000000 &  0.190616 & -0.384164 & -0.048327 & -0.033872 \\
        mass      &  -0.051003 &  0.093094 & -0.008223 &  0.102524 &  0.190616 &  1.000000 &  0.424990 &  0.195906 & -0.222011 \\
        radius    &   0.170720 & -0.092749 &  0.312863 & -0.133690 & -0.384164 &  0.424990 &  1.000000 &  0.213616 & -0.032948 \\
        M\_H       &   0.237106 & -0.099701 &  0.196941 & -0.099383 & -0.048327 &  0.195906 &  0.213616 &  1.000000 & -0.114388 \\
        C\_N       &  -0.074333 &  0.153920 & -0.105284 & -0.184950 & -0.033872 & -0.222011 & -0.032948 & -0.114388 &  1.000000 \\
        \bottomrule
        \end{tabular}
    \caption{Kendall correlation matrix of parameters checked for interdependence.}
\end{table*}


==> Giants_Corr.tex <==
\begin{table*}
    \centering
        \begin{tabular}{lrrrrrrr}
        \toprule
        {} &  NUV\_exess &     vsini &     psini &      mass &    radius &       M\_H &       C\_N \\
        \midrule
        NUV\_exess &   1.000000 & -0.435463 &  0.396239 & -0.051003 &  0.170720 &  0.237106 & -0.074333 \\
        vsini     &  -0.435463 &  1.000000 & -0.779886 &  0.093094 & -0.092749 & -0.099701 &  0.153920 \\
        psini     &   0.396239 & -0.779886 &  1.000000 & -0.008223 &  0.312863 &  0.196941 & -0.105284 \\
        mass      &  -0.051003 &  0.093094 & -0.008223 &  1.000000 &  0.424990 &  0.195906 & -0.222011 \\
        radius    &   0.170720 & -0.092749 &  0.312863 &  0.424990 &  1.000000 &  0.213616 & -0.032948 \\
        M\_H       &   0.237106 & -0.099701 &  0.196941 &  0.195906 &  0.213616 &  1.000000 & -0.114388 \\
        C\_N       &  -0.074333 &  0.153920 & -0.105284 & -0.222011 & -0.032948 & -0.114388 &  1.000000 \\
        \bottomrule
        \end{tabular}
    \caption{Kendall correlation matrix of parameters checked for interdependence.}
\end{table*}


==> Giants_Corr2_lg.tex <==
\begin{table*}
    \centering
    \begin{tabular}{lrrrrrrrrr}
    \toprule
    {} &  NUV Excess &  $v \sin i$ &  $P/\sin i$ &   $T_{\rm eff}$ &  $\log g$ &  mass &  radius &   [M/H] &   [C/N] \\
    \midrule
    NUV Excess &       1.00 &  -0.50 &   0.50 &  0.41 & -0.12 &  0.13 &    0.13 &  0.30 & -0.20 \\
    $v \sin i$     &      -0.50 &   1.00 &  -0.82 & -0.32 &  0.14 &  0.06 &    0.04 & -0.17 &  0.15 \\
    $P/\sin i$     &       0.50 &  -0.82 &   1.00 &  0.35 & -0.19 &  0.12 &    0.15 &  0.27 & -0.22 \\
    $T_{\rm eff}$         &       0.41 &  -0.32 &   0.35 &  1.00 &  0.08 &  0.20 &    0.17 &  0.11 & -0.25 \\
    $\log g$      &      -0.12 &   0.14 &  -0.19 &  0.08 &  1.00 & -0.14 &   -0.26 & -0.07 &  0.10 \\
    mass      &       0.13 &   0.06 &   0.12 &  0.20 & -0.14 &  1.00 &    0.88 &  0.36 & -0.15 \\
    radius    &       0.13 &   0.04 &   0.15 &  0.17 & -0.26 &  0.88 &    1.00 &  0.33 & -0.17 \\
    ${\rm [M/H]}$     &       0.30 &  -0.17 &   0.27 &  0.11 & -0.07 &  0.36 &    0.33 &  1.00 & -0.27 \\
    ${\rm [C/N]}$      &      -0.20 &   0.15 &  -0.22 & -0.25 &  0.10 & -0.15 &   -0.17 & -0.27 &  1.00 \\
    \bottomrule
    \end{tabular}
\end{table*}

==> Giants_Corr2_rc.tex <==
\begin{table*}
    \centering
    \begin{tabular}{lrrrrrrrrr}
    \toprule
    {} &  NUV Excess &  $v \sin i$ &  $P/\sin i$ &   $T_{\rm eff}$ &  $\log g$ &  mass &  radius &   [M/H] &   [C/N] \\
    \midrule
    NUV Excess &       1.00 &  -0.18 &   0.16 & -0.03 &  0.04 & -0.07 &   -0.08 &  0.19 & -0.16 \\
    $v \sin i$     &      -0.18 &   1.00 &  -0.88 &  0.03 &  0.17 &  0.00 &   -0.06 & -0.04 &  0.27 \\
    $P/\sin i$     &       0.16 &  -0.88 &   1.00 & -0.05 & -0.20 &  0.10 &    0.18 &  0.03 & -0.29 \\
    $T_{\rm eff}$         &      -0.03 &   0.03 &  -0.05 &  1.00 &  0.09 & -0.12 &   -0.20 & -0.24 &  0.02 \\
    $\log g$      &       0.04 &   0.17 &  -0.20 &  0.09 &  1.00 &  0.22 &   -0.10 &  0.24 & -0.04 \\
    mass      &      -0.07 &   0.00 &   0.10 & -0.12 &  0.22 &  1.00 &    0.68 &  0.14 & -0.19 \\
    radius    &      -0.08 &  -0.06 &   0.18 & -0.20 & -0.10 &  0.68 &    1.00 &  0.02 & -0.11 \\
    ${\rm [M/H]}$      &       0.19 &  -0.04 &   0.03 & -0.24 &  0.24 &  0.14 &    0.02 &  1.00 & -0.29 \\
    ${\rm [C/N]}$       &      -0.16 &   0.27 &  -0.29 &  0.02 & -0.04 & -0.19 &   -0.11 & -0.29 &  1.00 \\
    \bottomrule
    \end{tabular}
\end{table*}


==> Giants_Corr_Comp.tex <==
\begin{table*}
\centering
    \begin{tabular}{lrrrrrrr}
    \toprule
    {} &  NUV\_exess &     vsini &     psini &      mass &    radius &       M\_H &       C\_N \\
    \midrule
    NUV\_exess &   1.000000 & -0.372509 &  0.409771 & -0.081842 &  0.151751 &  0.266689 & -0.046493 \\
    vsini     &  -0.372509 &  1.000000 & -0.781493 &  0.099854 & -0.081504 & -0.140155 &  0.137003 \\
    psini     &   0.409771 & -0.781493 &  1.000000 & -0.016436 &  0.300011 &  0.195655 & -0.109648 \\
    mass      &  -0.081842 &  0.099854 & -0.016436 &  1.000000 &  0.427558 &  0.194641 & -0.216706 \\
    radius    &   0.151751 & -0.081504 &  0.300011 &  0.427558 &  1.000000 &  0.210289 & -0.029044 \\
    M\_H       &   0.266689 & -0.140155 &  0.195655 &  0.194641 &  0.210289 &  1.000000 & -0.232016 \\
    C\_N       &  -0.046493 &  0.137003 & -0.109648 & -0.216706 & -0.029044 & -0.232016 &  1.000000 \\
    \bottomrule
    \end{tabular}
\caption{Kendall correlation matrix of parameters checked for interdependence..}
\end{table*}


==> Giants_Param_Data.tex <==
\begin{table*}
    \centering
        \begin{tabular}{llrrrrrrrrrr}
            \toprule
            {} &           APOGEE\_ID &        $T_{\rm eff}$  &  $\log g$ &   $v \sin i$ &  $\sigma_{v\sin i}$ &    $J$ &  $\sigma_J$ &   $K_S$ &  $\sigma_{K_S}$ &   NUV &  $\sigma_{NUV}$ \\
            \midrule
            0  &  2M00013362+5549387 &  4768.57 &  3.09387 &   8.800779 &      0.759330 &   8.941 &   0.029 &  8.083 &   0.029 &  18.53321 &    0.086588 \\
            1  &  2M07354367-1059049 &  4638.21 &  2.36800 &   0.670641 &      0.948429 &   8.810 &   0.020 &  8.055 &   0.020 &  17.61304 &    0.028980 \\
            2  &  2M07360651+2114107 &  4798.02 &  3.04886 &   9.513528 &      0.375790 &   9.303 &   0.023 &  8.667 &   0.023 &  18.00905 &    0.034864 \\
            3  &  2M08111162+3255049 &  4772.47 &  2.44691 &   4.266745 &      1.557929 &   8.778 &   0.020 &  8.138 &   0.020 &  16.07101 &    0.004962 \\
            4  &  2M08363324+1516597 &  4537.72 &  3.06447 &  12.564625 &      0.091538 &   8.091 &   0.034 &  7.378 &   0.034 &  17.01466 &    0.032795 \\
            5  &  2M10513105-0103246 &  4624.71 &  3.17913 &  11.846786 &      0.498777 &   9.709 &   0.026 &  9.018 &   0.026 &  19.09305 &    0.020168 \\
            6  &  2M12031564+1606376 &  4231.16 &  3.28783 &  48.912584 &      4.559802 &   9.771 &   0.020 &  8.947 &   0.020 &  18.45735 &    0.012068 \\
            7  &  2M12091873+0023078 &  4846.49 &  3.12604 &   0.858732 &      1.214430 &   8.897 &   0.035 &  8.335 &   0.035 &  17.55636 &    0.037061 \\
            8  &  2M12440204-0716121 &  5052.72 &  3.21357 &   2.300090 &      1.627912 &   7.903 &   0.030 &  7.341 &   0.030 &  16.28543 &    0.005399 \\
            9  &  2M12474320-0712154 &  4387.52 &  3.09616 &  62.718866 &      8.324013 &  10.308 &   0.024 &  9.643 &   0.024 &  17.72204 &    0.046813 \\
            10 &  2M13230135+1259254 &  4623.59 &  3.29675 &  31.650773 &      7.227865 &  10.108 &   0.021 &  9.596 &   0.021 &  16.71942 &    0.025826 \\
            \bottomrule
        \end{tabular}
    \caption{Photometric and spectral data used to define NUV excess. The full table is available in the electronic journal; a portion is shown here for guidance regarding its format and content.
    {\bf [DON REDUCE ALL VALUES TO TWO SIG FIGS.]}}
\end{table*}


==> Giants_Params_Data.tex <==
\begin{table*}
    \centering
    \normalsize
        \begin{tabular}{lccccccccccc}
        \toprule
        {} &           APOGEE\_ID &        $T_{\rm eff}$  &  $\log g$ &   $v \sin i$ &  $\sigma_{v\sin i}$ &    $J$ &  $\sigma_J$ &   $K_S$ &  $\sigma_{K_S}$ &   NUV &  $\sigma_{NUV}$ \\
        \midrule
        0 &  2M00013362+5549387 &  4768.57 &  3.09 &   8.80 &       0.76 &   8.94 &  0.03 &   8.08 &  0.03 &  18.53 &   0.09 \\
        1 &  2M00080122+0128582 &  4984.84 &  3.17 &   1.73 &       1.23 &  11.29 &  0.03 &  10.67 &  0.03 &  20.08 &   0.03 \\
        2 &  2M00322120+8518390 &  4410.32 &  3.13 &  19.17 &       0.00 &  12.51 &  0.02 &  11.73 &  0.02 &  21.55 &   0.22 \\
        3 &  2M00421158+1710125 &  4308.45 &  3.27 &  33.76 &       3.15 &  12.34 &  0.03 &  11.59 &  0.03 &  21.21 &   0.16 \\
        4 &  2M00471103+1738040 &  3929.20 &  3.22 &  18.34 &       0.00 &  10.81 &  0.02 &   9.77 &  0.02 &  20.53 &   0.18 \\
        5 &  2M02133613+1305115 &  4156.57 &  2.40 &  15.74 &       0.75 &   8.60 &  0.03 &   7.68 &  0.03 &  20.07 &   0.07 \\
        6 &  2M04342218+5205307 &  4779.59 &  2.39 &   1.10 &       1.56 &  10.61 &  0.03 &   9.54 &  0.03 &  21.78 &   0.47 \\
        7 &  2M05010002+2254304 &  4393.18 &  3.20 &  11.24 &       1.23 &   9.81 &  0.02 &   8.93 &  0.02 &  21.31 &   0.11 \\
        8 &  2M05025805+4124468 &  4476.51 &  3.27 &  44.00 &       0.00 &  10.47 &  0.02 &   9.62 &  0.02 &  20.57 &   0.25 \\
        9 &  2M05170212+1702061 &  4411.45 &  3.08 &  55.71 &       0.00 &   9.83 &  0.02 &   9.04 &  0.02 &  18.52 &   0.04 \\
        \bottomrule
        \end{tabular}
    \caption{Photometric and spectral data used to define NUV excess. The full table is available in the electronic journal; a portion is shown here for guidance regarding its format and content.}
\end{table*}


==> Kendall_Corr_Final.tex <==
\begin{table*}
    \centering
        \def\arraystretch{1.5}
        \hspace*{-2.25cm}\begin{tabular}{lrrrrrrrrr}
        \toprule
        {} &  NUV exess &  $v \sin i$  &  $P_{rot}/ \sin i$ &    $T_{\rm eff}$ &  $\log g$ &  mass &  radius &   [M/H] &   [C/N] \\
        \midrule
        NUV exess &       1.00 &  -0.46 &    0.35 &  0.18 & -0.30 & -0.12 &    0.08 &  0.20 & -0.05 \\
        $v \sin i$     &      -0.46 &   1.00 &   -0.76 & -0.25 &  0.27 &  0.14 &   -0.01 & -0.10 &  0.12 \\
        $P_{rot}/ \sin i$    &       0.35 &  -0.76 &    1.00 & -0.15 & -0.41 & -0.04 &    0.25 &  0.17 & -0.08 \\
        $T_{\rm eff}$        &       0.18 &  -0.25 &   -0.15 &  1.00 &  0.12 &  0.10 &   -0.23 & -0.11 & -0.15 \\
        $\log g$      &      -0.30 &   0.27 &   -0.41 &  0.12 &  1.00 &  0.22 &   -0.35 & -0.05 & -0.06 \\
        mass      &      -0.12 &   0.14 &   -0.04 &  0.10 &  0.22 &  1.00 &    0.43 &  0.17 & -0.19 \\
        radius    &       0.08 &  -0.01 &    0.25 & -0.23 & -0.35 &  0.43 &    1.00 &  0.17 &  0.00 \\
        {[M/H]}       &       0.20 &  -0.10 &    0.17 & -0.11 & -0.05 &  0.17 &    0.17 &  1.00 & -0.11 \\
        {[C/N]}       &      -0.05 &   0.12 &   -0.08 & -0.15 & -0.06 & -0.19 &    0.00 & -0.11 &  1.00 \\
        \bottomrule
        \end{tabular}
    \caption{Kendall Tau correllation matrix for the 242 giants in our dataset, of which 172 have determined radii. }
\end{table*}



==> Kendall_Corr_Final_lg.tex <==
\begin{table*}
    \centering
        \def\arraystretch{1.5}
        \hspace*{-2.25cm}\begin{tabular}{lrrrrrrrrr}
        \toprule
        {} &  NUV exess &  $v \sin i$  &  $P_{rot}/ \sin i$ &    $T_{\rm eff}$ &  $\log g$ &  mass &  radius &   [M/H] &   [C/N] \\
        \midrule
        NUV exess &       1.00 &  -0.51 &    0.40 &  0.43 & -0.09 & -0.06 &   -0.07 &  0.09 & -0.08 \\
         $v \sin i$     &      -0.51 &   1.00 &   -0.80 & -0.41 &  0.09 &  0.19 &    0.18 & -0.02 &  0.11 \\
        $P_{rot}/ \sin i$    &       0.40 &  -0.80 &    1.00 &  0.22 & -0.12 & -0.01 &    0.02 &  0.26 & -0.14 \\
        $T_{\rm eff}$        &       0.43 &  -0.41 &    0.22 &  1.00 & -0.02 &  0.17 &    0.11 & -0.06 & -0.17 \\
        $\log g$      &      -0.09 &   0.09 &   -0.12 & -0.02 &  1.00 & -0.08 &   -0.21 &  0.03 &  0.08 \\
        mass      &      -0.06 &   0.19 &   -0.01 &  0.17 & -0.08 &  1.00 &    0.87 &  0.34 & -0.08 \\
        radius    &      -0.07 &   0.18 &    0.02 &  0.11 & -0.21 &  0.87 &    1.00 &  0.32 & -0.09 \\
        {[M/H]}       &       0.09 &  -0.02 &    0.26 & -0.06 &  0.03 &  0.34 &    0.32 &  1.00 & -0.04 \\
        {[C/N]}       &      -0.08 &   0.11 &   -0.14 & -0.17 &  0.08 & -0.08 &   -0.09 & -0.04 &  1.00 \\
        \bottomrule
        \end{tabular}
    \caption{Kendall Tau correllation matrix for the 123 RGB stars in our dataset, of which 62 have determined radii. }
\end{table*}

==> Kendall_Corr_Final_rc.tex <==
\begin{table*}
    \centering
        \def\arraystretch{1.5}
        \hspace*{-2.25cm}\begin{tabular}{lrrrrrrrrr}
        \toprule
        {} &  NUV exess &  $v \sin i$  &  $P_{rot}/ \sin i$ &    $T_{\rm eff}$ &  $\log g$ &  mass &  radius &   [M/H] &   [C/N] \\ \midrule
        NUV exess &       1.00 &  -0.28 &    0.18 &  0.02 &  0.08 & -0.03 &   -0.05 &  0.25 & -0.16 \\
        $v \sin i$     &      -0.28 &   1.00 &   -0.88 & -0.05 &  0.15 &  0.01 &   -0.05 & -0.08 &  0.23 \\
        $P_{rot}/ \sin i$    &       0.18 &  -0.88 &    1.00 & -0.04 & -0.23 &  0.10 &    0.17 &  0.04 & -0.29 \\
        $T_{\rm eff}$        &       0.02 &  -0.05 &   -0.04 &  1.00 &  0.10 & -0.11 &   -0.18 & -0.16 & -0.06 \\
        $\log g$      &       0.08 &   0.15 &   -0.23 &  0.10 &  1.00 &  0.21 &   -0.11 &  0.23 & -0.05 \\
        mass      &      -0.03 &   0.01 &    0.10 & -0.11 &  0.21 &  1.00 &    0.68 &  0.12 & -0.18 \\
        radius    &      -0.05 &  -0.05 &    0.17 & -0.18 & -0.11 &  0.68 &    1.00 &  0.00 & -0.10 \\
        {[M/H]}       &       0.25 &  -0.08 &    0.04 & -0.16 &  0.23 &  0.12 &    0.00 &  1.00 & -0.26 \\
        {[C/N]}      &      -0.16 &   0.23 &   -0.29 & -0.06 & -0.05 & -0.18 &   -0.10 & -0.26 &  1.00 \\
        \bottomrule
        \end{tabular}
    \caption{Kendall Tau correllation matrix for the 119 RC stars in our dataset, of which 110 have determined radii.}
\end{table*}



==> Params_Data_Final.tex <==
\begin{table*}
    \centering
        \begin{tabular}{llccccccccccc}
        \toprule
        {} &           APOGEE ID &  LOCATION ID &        $T_{\rm eff}$ &  $\log g$ &  $v\sin i$ &  $\sigma_{v\sin i}$ &      $J$ &   $\sigma_J$ &     $K_S$ &  $\sigma_{K_S}$ &    $NUV$ &  $\sigma_{NUV}$ \\
        \midrule
        {} &  2M08111162+3255049 &         4103 &  4772.47 &  2.45 &   4.27 &       1.56 &   8.78 &  0.02 &   8.14 &  0.02 &  16.17 &   0.02 \\
        {} &  2M10513105-0103246 &         4236 &  4624.71 &  3.18 &  11.85 &       0.50 &   9.71 &  0.03 &   9.02 &  0.03 &  19.09 &   0.02 \\
        {} &  2M20011221+5617287 &         4276 &  4861.04 &  3.20 &   0.76 &       1.07 &  11.81 &  0.02 &  11.15 &  0.02 &  21.50 &   0.26 \\
        {} &  2M15220704-0054481 &         4207 &  4468.82 &  3.09 &   1.15 &       1.63 &   9.70 &  0.02 &   8.91 &  0.02 &  19.82 &   0.10 \\
        {} &  2M07360651+2114107 &         4147 &  4798.02 &  3.05 &   9.51 &       0.38 &   9.30 &  0.02 &   8.67 &  0.02 &  18.01 &   0.03 \\
        {} &  2M00013362+5549387 &         4264 &  4768.57 &  3.09 &   8.80 &       0.76 &   8.94 &  0.03 &   8.08 &  0.03 &  18.53 &   0.09 \\
        {} &  2M11471494+0124506 &         4124 &  4763.45 &  3.25 &   1.07 &       1.51 &   9.31 &  0.02 &   8.70 &  0.02 &  18.79 &   0.02 \\
        {} &  2M08363324+1516597 &         4534 &  4537.72 &  3.06 &  12.56 &       0.09 &   8.09 &  0.03 &   7.38 &  0.03 &  17.01 &   0.03 \\
        {} &  2M18014184+6011596 &         4526 &  4843.05 &  3.23 &   3.66 &       2.71 &  11.99 &  0.02 &  11.43 &  0.02 &  19.88 &   0.10 \\
        {} &  2M12285832+1351453 &         4218 &  4622.74 &  3.15 &  11.04 &       0.86 &   9.85 &  0.02 &   9.20 &  0.02 &  18.80 &   0.02 \\
        \bottomrule
        \end{tabular}
    \caption{{Stellar parameters used to derive $NUV$ excess. The full table is provided in machine-readable form; a portion is shown here for guidance regarding its format and contents.}}\label{tab:data}
\end{table*}

